Diffusion Probabilistic Models for 3D Point Cloud Generation

We present a probabilistic model for point cloud generation, which is fundamental for various 3D vision tasks such as shape completion, upsampling, synthesis and data augmentation. Inspired by the diffusion process in non-equilibrium thermodynamics, we view points in point clouds as particles in a thermodynamic system in contact with a heat bath, which diffuse from the original distribution to a noise distribution. Point cloud generation thus amounts to learning the reverse diffusion process that transforms the noise distribution to the distribution of a desired shape. Specifically, we propose to model the reverse diffusion process for point clouds as a Markov chain conditioned on certain shape latent. We derive the variational bound in closed form for training and provide implementations of the model. Experimental results demonstrate that our model achieves competitive performance in point cloud generation and auto-encoding. The code is available at \url{https://github.com/luost26/diffusion-point-cloud}.

==> figures/algorithm-simp.tex <==
\algrenewcommand\algorithmicindent{1.0em}%
\begin{algorithm}[H]
  \caption{Training (Simplified)} \label{alg:trainingsimp}
  \small
  \begin{algorithmic}[1]
    \Repeat
      \State Sample $\mX^\ts{0} \sim q_\mathrm{data}(\mX^\ts{0})$
      \State Sample $\vz \sim q_\vphi(\vz | \mX^\ts{0})$
      \State Sample $t \sim \operatorname{Uniform}(\{ 1, \ldots, T\})$
      \State Sample $\vepsilon \sim \mathcal{N}(\vzero, \mI)$
      \State Compute $\nabla \big[  \sum_{i=1}^{N} \| \vepsilon - \vepsilon_\vtheta( \sqrt{\bar{\alpha}_t} \vx_i^\ts{0} + \sqrt{1 - \bar{\alpha}_t} \vepsilon, t , \vz) \|^2  -  \frac{1}{T} \KL( q_\vphi(\vz | \mX^\ts{0}) \| p(\vz) \big] $; Then perform gradient descent.
    \Until{converged}
  \end{algorithmic}
\end{algorithm}


==> figures/algorithms.tex <==
\algrenewcommand\algorithmicindent{0.5em}%
\begin{figure}[H] % [t] for being fixed at the top of the page
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
  \caption{Training} \label{alg:training}
  \small
  \begin{algorithmic}[1]
    \Repeat
      \State Sample $\mX^\ts{0} \sim q_\mathrm{data}(\mX^\ts{0})$
      \State Sample $\vz \sim q_\vphi(\vz | \mX^\ts{0})$
      \For{$t = 1 \ldots T$}
        \State Sample $\mX^\ts{t} \sim q(\mX^\ts{t} | \mX^\ts{t-1})$
      \EndFor
      \State Compute $\nabla L_G(\vtheta, \vphi, \valpha)$ using samples $\mX^\ts{0:T}$ and $\vz$; Then perform gradient descent.
    \Until{converged}
  \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
  \caption{Sampling} \label{alg:sampling}
  \small
  \begin{algorithmic}[1]
    \vspace{.15in}
    \State Sample $\vw \sim \mathcal{N}(\vzero, \mI)$
    \State $\vz \gets F_\valpha(\vw)$
    \State $\mX^\ts{T} \gets \{ \vx_i^\ts{T} \} \sim \mathcal{N}(\vzero, \mI)$
    \For{$t = T \ldots 1$}
      \State Sample $\mX^\ts{t-1} \sim p_\vtheta(\mX^\ts{t-1} | \mX^\ts{t}, \vz)$
    \EndFor
    \State \Return $\mX^\ts{0}$
    \vspace{.15in}
  \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-1em}
\end{figure}

==> others/others.tex <==
\section{Evaluation Metrics}
\label{app:metrics}

\begin{equation}
    \operatorname{CD}(\mX, \mY) = \frac{1}{|\mX|}\sum_{\vx \in \mX} \min_{\vy \in \mY} \| \vx - \vy \|_2^2 + \frac{1}{\mY}\sum_{\vy \in \mY} \min_{\vx \in \mX} \| \vy - \vx \|_2^2,
\end{equation}

\begin{equation}
    \operatorname{EMD}(\mX, \mY) = \min_{\phi:\mX \rightarrow \mY} \frac{1}{|\mX|} \sum_{\vx \in \mX} \| \vx - \phi(\vx)\|_2,
\end{equation}

\begin{equation}
    \operatorname{MMD}\left(\gS_{g}, \gS_{r}\right)=\frac{1}{\left|\gS_{r}\right|} \sum_{\mY \in \gS_{r}} \min _{\mX \in \gS_{g}} D(\mX, \mY),
\end{equation}

\begin{equation}
    \operatorname{COV}\left(\gS_{g}, \gS_{r}\right) =  \frac{1}{\left|\gS_{r}\right|} \big|\big\{\arg \min _{\mY \in \gS_{r}} D(\mX, \mY) \big| \mX \in \gS_{g}\big\}\big|,
\end{equation}

\begin{equation}
    \operatorname{1-NNA} \left(\gS_{g}, \gS_{r}\right) = \frac{\sum_{\mX \in \gS_{g}} \mathbb{I}\left[\mN_{\mX} \in \gS_{g}\right]+\sum_{\mY \in \gS_{r}} \mathbb{I}\left[\mN_{\mY} \in \gS_{r}\right]}{\left|\gS_{g}\right|+\left|\gS_{r}\right|}
\end{equation}

